IOTLB-SC: An Accelerator-Independent Leakage Source in Modern Cloud Systems

Hardware peripherals such as GPUs and FPGAs are commonly available in server-grade computing to accelerate specific compute tasks, from database queries to machine learning. CSPs have integrated these accelerators into their infrastructure and let tenants combine and configure these components flexibly, based on their needs. Securing I/O interfaces is critical to ensure proper isolation between tenants in these highly complex, heterogeneous, yet shared server systems, especially in the cloud, where some peripherals may be under control of a malicious tenant. In this work, we investigate the interfaces that connect peripheral hardware components to each other and the rest of the system.We show that the I/O memory management units (IOMMUs) - intended to ensure proper isolation of peripherals - are the source of a new attack surface: the I/O translation look-aside buffer (IOTLB). We show that by using an FPGA accelerator card one can gain precise information over IOTLB activity. That information can be used for covert communication between peripherals without bothering CPU or to directly extract leakage from neighboring accelerated compute jobs such as GPU-accelerated databases. We present the first qualitative and quantitative analysis of this newly uncovered attack surface before fine-grained channels become widely viable with the introduction of CXL and PCIe 5.0. In addition, we propose possible countermeasures that software developers, hardware designers, and system administrators can use to suppress the observed side-channel leakages and analyze their implicit costs.

==> figures/evsets/evset_count_a10l_flush.tex <==
\pgfplotsset{
    BlueBars/.style={
        draw=plotblue,
        fill=plotblue,
        bar width=0.25
    },
}
\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_count_f1_r0_s0_a10.csv}\rzsz
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_count_f1_r1_s0_a10.csv}\rosz
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_count_f1_r0_s1_a10.csv}\rzso
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_count_f1_r1_s1_a10.csv}\roso
\begin{tikzpicture}
\begin{axis} [
        name=mode0,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        % ymin=1,
        % ymax=35,
        xmin=-1,
        xmax=5,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={(\#Clock Cycles)},
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rzsz};
    
    \node[draw,fill=white,anchor=north west] (m0) at (rel axis cs: 0,1) {(a)};
    % \node[anchor=south east] (thresh0) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode1,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        % ymin=1,
        % ymax=35,
        xmin=-1,
        xmax=5,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(mode0.east) + (.75cm,0cm)$)},
        anchor=west,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rosz};
    
    \node[draw,fill=white,anchor=north west] (m1) at (rel axis cs: 0,1) {(b)};
    % \node[anchor=south east] (thresh1) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode2,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        % ymin=1,
        % ymax=35,
        xmin=-1,
        xmax=5,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency},
        at={($(mode0.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rzso};
    
    \node[draw,fill=white,anchor=north west] (m2) at (rel axis cs: 0,1) {(c)};
    % \node[anchor=south east] (thresh2) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode3,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        % ymin=1,
        % ymax=35,
        xmin=-1,
        xmax=5,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(mode1.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\roso};
    
    \node[draw,fill=white,anchor=north west] (m3) at (rel axis cs: 0,1) {(d)};
    % \node[anchor=south east] (thresh3) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\path (mode2.south) -- node[midway,below,yshift=-.625cm] {\#Eviction Sets} (mode3.south);
\path (mode0.west) -- node[midway,above,rotate=90,yshift=.75cm] {Frequency} (mode2.west);
\end{tikzpicture}


==> figures/evsets/evset_count_a10v.tex <==
\pgfplotsset{
    BlueBars/.style={
        draw=plotblue,
        fill=plotblue,
        bar width=0.25
    },
}
\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_count_r0_s0_a10.csv}\rzsz
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_count_r1_s0_a10.csv}\rosz
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_count_r0_s1_a10.csv}\rzso
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_count_r1_s1_a10.csv}\roso
\begin{tikzpicture}
\begin{axis} [
        name=mode0,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=1,
        ymax=35,
        xmin=5,
        xmax=45,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={(\#Clock Cycles)},
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rzsz};
    
    \node[draw,fill=white,anchor=north west] (m0) at (rel axis cs: 0,1) {(a)};
    % \node[anchor=south east] (thresh0) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode1,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=1,
        ymax=35,
        xmin=5,
        xmax=45,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(mode0.east) + (.75cm,0cm)$)},
        anchor=west,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rosz};
    
    \node[draw,fill=white,anchor=north west] (m1) at (rel axis cs: 0,1) {(b)};
    % \node[anchor=south east] (thresh1) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode2,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=1,
        ymax=35,
        xmin=5,
        xmax=45,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency},
        at={($(mode0.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rzso};
    
    \node[draw,fill=white,anchor=north west] (m2) at (rel axis cs: 0,1) {(c)};
    % \node[anchor=south east] (thresh2) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode3,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=1,
        ymax=35,
        xmin=5,
        xmax=45,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(mode1.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\roso};
    
    \node[draw,fill=white,anchor=north west] (m3) at (rel axis cs: 0,1) {(d)};
    % \node[anchor=south east] (thresh3) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\path (mode2.south) -- node[midway,below,yshift=-.625cm] {\#Eviction Sets} (mode3.south);
\path (mode0.west) -- node[midway,above,rotate=90,yshift=.75cm] {Frequency} (mode2.west);
\end{tikzpicture}


==> figures/evsets/evset_count_s10v.tex <==
\begin{axis} [
        name=modec0,
        ybar,
        bar width=.1,
        height=3cm,
        width=.275\linewidth,
        ymin=1,
        ymax=35,
        xmin=5,
        xmax=45,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={(\#Clock Cycles)},
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\crzsz};
    
    \node[draw,fill=white,anchor=north west] (mc0) at (rel axis cs: 0,1) {(Ca)};
    % \node[anchor=south east] (threshc0) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (threshc0.south east);
\end{axis}

\begin{axis} [
        name=modec1,
        ybar,
        bar width=.1,
        height=3cm,
        width=.275\linewidth,
        ymin=1,
        ymax=35,
        xmin=5,
        xmax=45,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(modec0.east) + (.75cm,0cm)$)},
        anchor=west,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\crosz};
    
    \node[draw,fill=white,anchor=north west] (mc1) at (rel axis cs: 0,1) {(Cb)};
    % \node[anchor=south east] (threshc1) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (threshc0.south east);
\end{axis}

\begin{axis} [
        name=modec2,
        ybar,
        bar width=.1,
        height=3cm,
        width=.275\linewidth,
        ymin=1,
        ymax=35,
        xmin=5,
        xmax=45,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency},
        at={($(modec0.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\crzso};
    
    \node[draw,fill=white,anchor=north west] (mc2) at (rel axis cs: 0,1) {(Cc)};
    % \node[anchor=south east] (threshc2) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (threshc0.south east);
\end{axis}

\begin{axis} [
        name=modec3,
        ybar,
        bar width=.1,
        height=3cm,
        width=.275\linewidth,
        ymin=1,
        ymax=35,
        xmin=5,
        xmax=45,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(modec1.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\croso};
    
    \node[draw,fill=white,anchor=north west] (mc3) at (rel axis cs: 0,1) {(Cd)};
    % \node[anchor=south east] (threshc3) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (threshc0.south east);
\end{axis}

\path (modec2.south) -- node[midway,below,yshift=-.5cm]          {\#Eviction Sets}                                    (modec3.south);
\path (modec0.west)  -- node[midway,above,rotate=90,yshift=.5cm] {Number of Occurrences}                              (modec2.west) ;
\path (modec0.north) -- node[midway,above,yshift=.125cm]         {\bfseries Distributions of Number of Eviction Sets} (modec1.north);

==> figures/evsets/evset_size_a10l_flush.tex <==
\pgfplotsset{
    BlueBars/.style={
        draw=plotblue,
        fill=plotblue,
        bar width=0.25
    },
}
\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_size_f1_r0_s0_a10.csv}\rzsz
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_size_f1_r1_s0_a10.csv}\rosz
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_size_f1_r0_s1_a10.csv}\rzso
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_size_f1_r1_s1_a10.csv}\roso
\begin{tikzpicture}
\begin{axis} [
        name=mode0,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=0,
        ymax=110,
        xmin=75,
        xmax=150,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={(\#Clock Cycles)},
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rzsz};
    
    \node[draw,fill=white,anchor=north west] (m0) at (rel axis cs: 0,1) {(a)};
    % \node[anchor=south east] (thresh0) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode1,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=0,
        ymax=110,
        xmin=75,
        xmax=150,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(mode0.east) + (.75cm,0cm)$)},
        anchor=west,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rosz};
    
    \node[draw,fill=white,anchor=north west] (m1) at (rel axis cs: 0,1) {(b)};
    % \node[anchor=south east] (thresh1) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode2,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=0,
        ymax=110,
        xmin=75,
        xmax=150,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency},
        at={($(mode0.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rzso};
    
    \node[draw,fill=white,anchor=north west] (m2) at (rel axis cs: 0,1) {(c)};
    % \node[anchor=south east] (thresh2) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode3,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=0,
        ymax=110,
        xmin=75,
        xmax=150,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(mode1.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\roso};
    
    \node[draw,fill=white,anchor=north west] (m3) at (rel axis cs: 0,1) {(d)};
    % \node[anchor=south east] (thresh3) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\path (mode2.south) -- node[midway,below,yshift=-.625cm] {Eviction Set Size} (mode3.south);
\path (mode0.west) -- node[midway,above,rotate=90,yshift=.75cm] {Frequency} (mode2.west);
\end{tikzpicture}


==> figures/evsets/evset_size_a10v.tex <==
\pgfplotsset{
    BlueBars/.style={
        draw=plotblue,
        fill=plotblue,
        bar width=0.25
    },
}
\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_size_r0_s0_a10.csv}\rzsz
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_size_r1_s0_a10.csv}\rosz
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_size_r0_s1_a10.csv}\rzso
\pgfplotstableread[col sep=comma,]{figures/evsets/data/evset_size_r1_s1_a10.csv}\roso
\begin{tikzpicture}
\begin{axis} [
        name=mode0,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=1,
        ymax=1750,
        xmin=10,
        xmax=30,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={(\#Clock Cycles)},
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rzsz};
    
    \node[draw,fill=white,anchor=north west] (m0) at (rel axis cs: 0,1) {(a)};
    % \node[anchor=south east] (thresh0) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode1,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=1,
        ymax=130,
        xmin=75,
        xmax=135,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(mode0.east) + (.75cm,0cm)$)},
        anchor=west,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rosz};
    
    \node[draw,fill=white,anchor=north west] (m1) at (rel axis cs: 0,1) {(b)};
    % \node[anchor=south east] (thresh1) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode2,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=1,
        ymax=1750,
        xmin=10,
        xmax=30,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency},
        at={($(mode0.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\rzso};
    
    \node[draw,fill=white,anchor=north west] (m2) at (rel axis cs: 0,1) {(c)};
    % \node[anchor=south east] (thresh2) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\begin{axis} [
        name=mode3,
        ybar,
        bar width=.1,
        height=4cm,
        width=.5\linewidth,
        ymin=1,
        ymax=130,
        xmin=75,
        xmax=135,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(mode1.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\roso};
    
    \node[draw,fill=white,anchor=north west] (m3) at (rel axis cs: 0,1) {(d)};
    % \node[anchor=south east] (thresh3) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (thresh0.south east);
\end{axis}

\path (mode2.south) -- node[midway,below,yshift=-.625cm] {Eviction Set Size} (mode3.south);
\path (mode0.west) -- node[midway,above,rotate=90,yshift=.75cm] {Frequency} (mode2.west);
\end{tikzpicture}


==> figures/evsets/evset_size_s10v.tex <==
\begin{axis} [
        name=modes0,
        ybar,
        bar width=.1,
        height=3cm,
        width=.275\linewidth,
        ymin=1,
        ymax=1450,
        xmin=10,
        xmax=30,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={(\#Clock Cycles)},
        at={($(modec1.east) + (+2.0cm,0cm)$)},
        anchor=west,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\srzsz};
    
    \node[draw,fill=white,anchor=north west] (ms0) at (rel axis cs: 0,1) {(Sa)};
    % \node[anchor=south east] (threshs0) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (threshs0.south east);
\end{axis}

\begin{axis} [
        name=modes1,
        ybar,
        bar width=.1,
        height=3cm,
        width=.275\linewidth,
        ymin=1,
        ymax=130,
        xmin=75,
        xmax=135,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(modes0.east) + (.75cm,0cm)$)},
        anchor=west,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\srosz};
    
    \node[draw,fill=white,anchor=north west] (ms1) at (rel axis cs: 0,1) {(Sb)};
    % \node[anchor=south east] (threshs1) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (threshs0.south east);
\end{axis}

\begin{axis} [
        name=modes2,
        ybar,
        bar width=.1,
        height=3cm,
        width=.275\linewidth,
        ymin=1,
        ymax=1450,
        xmin=10,
        xmax=30,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency},
        at={($(modes0.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\srzso};
    
    \node[draw,fill=white,anchor=north west] (ms2) at (rel axis cs: 0,1) {(Sc)};
    % \node[anchor=south east] (threshs2) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (threshs0.south east);
\end{axis}

\begin{axis} [
        name=modes3,
        ybar,
        bar width=.1,
        height=3cm,
        width=.275\linewidth,
        ymin=1,
        ymax=130,
        xmin=75,
        xmax=135,
        % xticklabels={,,},
        % xlabel={Eviction Set Address},
        % yticklabels={,,},
        % ylabel={Latency (\#Clock Cycles)},
        at={($(modes1.south) + (0cm,-.75cm)$)},
        anchor=north,
    ]
    \addplot[BlueBars] [
        select coords between index={0}{45}
    ] table [
        x=x, y=y, col sep=comma
    ] {\sroso};
    
    \node[draw,fill=white,anchor=north west] (ms3) at (rel axis cs: 0,1) {(Sd)};
    % \node[anchor=south east] (threshs3) at (axis cs: 123,200) {Threshold};
    % \draw[-,dashed] (axis cs: -7,200) -- (threshs0.south east);
\end{axis}

\path (modes2.south) -- node[midway,below,yshift=-.5cm]           {Eviction Set Size}                                (modes3.south);
\path (modes0.west)  -- node[midway,above,rotate=90,yshift=.75cm] {Number of Occurrences}                            (modes2.west) ;
\path (modes0.north) -- node[midway,above,yshift=.125cm]          {\bfseries Distributions of Size of Eviction Sets} (modes1.north);


==> figures/fingerprint_preproc_subfigs/subfig10.tex <==
\begin{tikzpicture}
\begin{axis}[%
scale only axis, width=0pt, height=0pt, hide axis,
point meta min=-1.28770935535431,
point meta max=1.01353704929352,
colormap/hot2,
colorbar horizontal,
colorbar style={
width=.95\linewidth%,
%at=(.5\linewidth,0)
}
]%
\addplot [draw=none] coordinates {(0,0)};
\end{axis}
\end{tikzpicture}

==> figures/iotlb_sets_ways/a10l_step1_directmapping_directaccessshape.tex <==
\begin{axis}[%
        name=dirdir,
        width=.35\linewidth,
        height=.2625\linewidth,
        scale only axis,
        point meta min=150,
        point meta max=300,
        % xmin=-1,
        % xmax=10,
        xtick={0.5,1.5,...,9.5},
        xticklabels={1,2,4,8,16,32,64,128,256},
        xticklabel style={rotate=90},
        % xlabel={Sets},
        % xlabel shift=-5pt,
        % ymin=0,
        % ymax=36,
        % ytick={\empty},
        ylabel={Ways},
        axis background/.style={fill=white},
        title style={font=\bfseries,align=center,text width=.3\linewidth,yshift=-5pt},
        title={Direct Mapping Direct Access}
    ]

    \addplot[%
        surf,
        shader=flat,
        colormap/hot2,
        mesh/rows=10,
    ] table[
        col sep=comma,
        point meta=\thisrow{d}
    ] {
x,y,d
0,1,165.594
0,2,165.5635
0,3,165.65233333333333
0,4,165.73025
0,5,165.8746
0,6,165.8458333333333
0,7,165.75285714285715
0,8,166.18625
0,9,165.80633333333333
0,10,166.0015
0,11,166.25809090909092
0,12,163.72725
0,13,164.17784615384616
0,14,166.28785714285715
0,15,166.30093333333335
0,16,166.2181875
0,17,166.2790588235294
0,18,165.0735
0,19,166.2727894736842
0,20,166.2426
0,21,162.32466666666662
0,22,162.05713636363635
0,23,166.33434782608697
0,24,166.20325
0,25,159.99784000000002
0,26,166.25165384615386
0,27,166.07396296296298
0,28,166.137
0,29,166.19741379310344
0,30,166.0899
0,31,166.23112903225805
0,32,166.29746875
0,33,166.24515151515152
0,34,166.2214705882353
0,35,165.2113714285714
1,1,165.889
1,2,165.5355
1,3,158.382
1,4,164.61925
1,5,165.77
1,6,166.2145
1,7,166.09671428571428
1,8,166.18675
1,9,166.35833333333335
1,10,166.2726
1,11,166.1021818181818
1,12,166.13608333333335
1,13,166.25369230769232
1,14,166.23185714285717
1,15,166.22920000000002
1,16,166.1905
1,17,166.2995294117647
1,18,166.24544444444444
1,19,166.2683157894737
1,20,166.25279999999998
1,21,166.17828571428575
1,22,166.22177272727274
1,23,166.14382608695655
1,24,162.20641666666666
1,25,162.98356
1,26,166.20446153846157
1,27,166.16185185185185
1,28,166.20128571428572
1,29,166.27486206896552
1,30,166.08610000000002
1,31,166.13512903225805
1,32,166.3115
1,33,166.24860606060605
1,34,166.25605882352943
1,35,166.26017142857143
2,1,163.976
2,2,158.1825
2,3,161.19566666666668
2,4,165.943
2,5,166.19940000000003
2,6,166.06933333333333
2,7,166.17042857142857
2,8,166.011
2,9,158.1938888888889
2,10,158.17659999999998
2,11,165.31690909090912
2,12,166.1099166666667
2,13,165.51761538461537
2,14,165.527
2,15,165.95073333333335
2,16,163.9765625
2,17,164.03935294117645
2,18,162.1921111111111
2,19,163.0683684210526
2,20,161.7165
2,21,160.15752380952378
2,22,160.3223181818182
2,23,165.04439130434784
2,24,164.594375
2,25,161.89448000000002
2,26,163.50230769230768
2,27,163.06966666666665
2,28,161.00817857142857
2,29,160.35306896551722
2,30,163.95253333333332
2,31,165.10338709677418
2,32,168.93784375
2,33,168.89818181818183
2,34,170.7858529411765
2,35,170.82374285714283
3,1,160.049
3,2,160.027
3,3,160.5066666666667
3,4,160.21775
3,5,160.11339999999998
3,6,160.1053333333333
3,7,160.4002857142857
3,8,160.285625
3,9,160.31522222222222
3,10,160.4398
3,11,160.2948181818182
3,12,160.24108333333334
3,13,160.44515384615386
3,14,161.8060714285714
3,15,165.3793333333333
3,16,171.2015
3,17,172.44735294117643
3,18,174.1986111111111
3,19,176.74563157894735
3,20,179.12625
3,21,181.27885714285716
3,22,183.11104545454546
3,23,184.58152173913044
3,24,189.23083333333332
3,25,188.09892000000002
3,26,190.56853846153848
3,27,190.55514814814813
3,28,191.80453571428572
3,29,193.0459655172414
3,30,194.0618333333333
3,31,194.88812903225806
3,32,195.84603125
3,33,196.63248484848486
3,34,197.4555
3,35,198.20302857142855
4,1,160.909
4,2,160.016
4,3,160.25533333333334
4,4,160.3495
4,5,160.3986
4,6,160.3371666666667
4,7,160.25657142857142
4,8,169.183625
4,9,173.92111111111112
4,10,178.95829999999998
4,11,183.10136363636366
4,12,186.87016666666668
4,13,189.78515384615383
4,14,191.83121428571425
4,15,194.04373333333334
4,16,195.8618125
4,17,197.39911764705886
4,18,198.85805555555555
4,19,200.2925263157895
4,20,201.4242
4,21,202.39671428571427
4,22,203.35968181818183
4,23,205.1005652173913
4,24,204.98820833333335
4,25,211.06304
4,26,208.88803846153843
4,27,207.0125925925926
4,28,207.55121428571428
4,29,208.15527586206898
4,30,208.61353333333332
4,31,209.1350322580645
4,32,209.4778125
4,33,210.64366666666666
4,34,210.75317647058824
4,35,210.71991428571428
5,1,159.964
5,2,160.09
5,3,160.352
5,4,175.47075
5,5,185.01160000000002
5,6,191.1233333333333
5,7,195.83485714285715
5,8,199.898375
5,9,202.14644444444443
5,10,204.32129999999998
5,11,205.65672727272727
5,12,207.039
5,13,208.20669230769232
5,14,209.63607142857143
5,15,210.56273333333334
5,16,211.40075
5,17,211.99064705882353
5,18,212.74022222222223
5,19,213.295
5,20,213.7393
5,21,214.03876190476188
5,22,214.60618181818182
5,23,214.875
5,24,215.21925
5,25,215.52496000000002
5,26,215.91657692307692
5,27,216.114
5,28,216.4352142857143
5,29,216.746
5,30,216.82946666666666
5,31,217.16045161290322
5,32,217.34603125
5,33,218.11987878787878
5,34,219.0373823529412
5,35,219.2617142857143
6,1,159.893
6,2,190.4315
6,3,201.3216666666667
6,4,207.428
6,5,209.645
6,6,212.29933333333332
6,7,213.53757142857143
6,8,214.87775
6,9,215.88833333333332
6,10,216.6765
6,11,217.18063636363635
6,12,217.63583333333332
6,13,219.74630769230768
6,14,218.46571428571428
6,15,219.95953333333333
6,16,220.91125
6,17,219.3354705882353
6,18,219.66094444444443
6,19,219.66805263157897
6,20,219.74044999999998
6,21,220.16495238095237
6,22,220.07059090909092
6,23,220.3641304347826
6,24,220.3981666666667
6,25,220.5276
6,26,220.90923076923076
6,27,220.87074074074073
6,28,220.98175
6,29,221.0726551724138
6,30,221.62453333333332
6,31,221.20606451612903
6,32,221.32375
6,33,221.284
6,34,221.36876470588234
6,35,221.58208571428574
7,1,221.053
7,2,221.886
7,3,222.318
7,4,222.04775
7,5,222.2216
7,6,222.3201666666667
7,7,222.61371428571428
7,8,222.969375
7,9,222.698
7,10,222.72190000000003
7,11,224.25990909090908
7,12,222.83833333333334
7,13,222.82638461538463
7,14,231.912
7,15,232.59346666666667
7,16,223.800625
7,17,223.92217647058823
7,18,223.01472222222222
7,19,223.2184736842105
7,20,223.24085
7,21,223.63
7,22,223.14836363636365
7,23,223.33217391304348
7,24,223.380625
7,25,223.41208
7,26,228.90638461538464
7,27,229.43274074074074
7,28,228.72396428571426
7,29,229.33568965517242
7,30,228.81983333333335
7,31,229.10409677419355
7,32,226.98571875
7,33,224.40151515151513
7,34,223.4110294117647
7,35,224.80457142857142
8,1,228.836
8,2,232.931
8,3,225.47033333333334
8,4,222.9945
8,5,222.25279999999998
8,6,225.3336666666667
8,7,225.70885714285714
8,8,223.275
8,9,226.251
8,10,223.05290000000002
8,11,226.40754545454544
8,12,223.02975
8,13,226.08315384615383
8,14,225.29142857142858
8,15,225.463
8,16,225.5074375
8,17,224.7119411764706
8,18,224.66705555555555
8,19,224.44784210526316
8,20,224.0945
8,21,223.28280952380953
8,22,224.19536363636362
8,23,223.41986956521737
8,24,223.43516666666662
8,25,223.47912
8,26,223.4618076923077
8,27,223.6504074074074
8,28,223.39214285714283
8,29,223.5740344827586
8,30,223.31473333333335
8,31,223.43006451612902
8,32,223.3870625
8,33,223.45915151515152
8,34,223.33920588235296
8,35,223.37462857142856
9,1,221.613
9,2,220.9115
9,3,222.6976666666667
9,4,222.31425
9,5,223.1362
9,6,223.427
9,7,223.24214285714285
9,8,223.53275
9,9,223.2783333333333
9,10,222.92100000000002
9,11,222.86163636363636
9,12,223.25241666666668
9,13,223.35023076923076
9,14,223.29178571428568
9,15,223.15586666666664
9,16,223.4410625
9,17,223.16576470588234
9,18,222.9491111111111
9,19,223.15694736842107
9,20,223.30385
9,21,223.34604761904762
9,22,223.22281818181818
9,23,223.2065652173913
9,24,223.19283333333334
9,25,223.19544
9,26,223.47330769230769
9,27,223.29281481481482
9,28,224.6883214285714
9,29,223.3872068965517
9,30,223.49073333333334
9,31,223.25832258064514
9,32,223.825375
9,33,223.72551515151514
9,34,223.4550294117647
9,35,223.29762857142856
        };
\end{axis}


==> figures/iotlb_sets_ways/a10l_step1_directmapping_randomaccessshape.tex <==
\begin{axis}[%
        name=dirrand,
        at={($(dirdir.south) + (0cm,-1.75cm)$)},
        anchor=north,
        width=.35\linewidth,
        height=.2625\linewidth,
        scale only axis,
        point meta min=150,
        point meta max=300,
        % xmin=-1,
        % xmax=10,
        xtick={0.5,1.5,...,9.5},
        xticklabels={1,2,4,8,16,32,64,128,256},
        xticklabel style={rotate=90},
        % xlabel={Sets},
        % xlabel shift=-5pt,
        % ymin=0,
        % ymax=36,
        % ytick={\empty},
        ylabel={Ways},
        axis background/.style={fill=white},
        title style={font=\bfseries,align=center,text width=.3\linewidth,yshift=-5pt},
        title={Direct Mapping Random Access},
    ]

    \addplot[%
        surf,
        shader=flat,
        colormap/hot2,
        mesh/rows=10,
    ] table[
        col sep=comma,
        point meta=\thisrow{d}
    ] {
x,y,d
0,1,165.531
0,2,165.852
0,3,165.94133333333332
0,4,165.883
0,5,165.931
0,6,165.91533333333334
0,7,166.1984285714286
0,8,165.99325
0,9,165.92644444444443
0,10,166.2216
0,11,165.99363636363637
0,12,166.01
0,13,166.00253846153845
0,14,166.07985714285712
0,15,166.10433333333333
0,16,166.0531875
0,17,166.0965882352941
0,18,166.123
0,19,164.32615789473687
0,20,161.95775
0,21,166.08280952380952
0,22,166.06736363636364
0,23,166.04526086956523
0,24,166.0404583333333
0,25,166.16944
0,26,165.934
0,27,166.02444444444444
0,28,165.9964642857143
0,29,166.13727586206892
0,30,166.09616666666668
0,31,166.09348387096773
0,32,166.158875
0,33,166.05148484848485
0,34,166.08344117647061
0,35,166.16202857142858
1,1,163.954
1,2,159.347
1,3,164.286
1,4,165.93675
1,5,165.9532
1,6,165.7798333333333
1,7,165.96971428571425
1,8,165.970125
1,9,166.048
1,10,165.7979
1,11,165.9949090909091
1,12,165.8224166666667
1,13,165.96353846153846
1,14,165.83621428571428
1,15,166.19240000000002
1,16,165.933375
1,17,166.0644705882353
1,18,166.01294444444443
1,19,166.02873684210527
1,20,166.04375
1,21,166.11809523809524
1,22,164.56754545454547
1,23,165.99808695652172
1,24,166.140375
1,25,166.08391999999998
1,26,166.05576923076922
1,27,166.07822222222222
1,28,166.07835714285716
1,29,166.1125172413793
1,30,166.13456666666664
1,31,166.1538387096774
1,32,166.11478125
1,33,166.1026060606061
1,34,166.15379411764704
1,35,166.11057142857143
2,1,164.224
2,2,162.8725
2,3,165.973
2,4,165.863
2,5,165.7138
2,6,165.80583333333334
2,7,165.96114285714287
2,8,166.10275
2,9,166.11944444444444
2,10,166.0254
2,11,166.24381818181817
2,12,166.0326666666667
2,13,166.17176923076926
2,14,166.0749285714286
2,15,166.20346666666669
2,16,166.183625
2,17,166.25811764705884
2,18,166.2326111111111
2,19,166.1382105263158
2,20,166.17755
2,21,166.19490476190475
2,22,166.0688181818182
2,23,166.1592173913043
2,24,166.139
2,25,166.13108000000003
2,26,164.09661538461538
2,27,166.22218518518517
2,28,166.20103571428572
2,29,166.15479310344827
2,30,168.3429
2,31,170.6065161290323
2,32,172.47284375
2,33,174.42048484848488
2,34,176.10408823529409
2,35,176.23542857142857
3,1,158.328
3,2,158.1145
3,3,163.5353333333333
3,4,165.97575
3,5,165.7798
3,6,165.5975
3,7,165.8675714285714
3,8,162.473125
3,9,158.14822222222224
3,10,158.39939999999999
3,11,165.99281818181817
3,12,165.958
3,13,165.92046153846155
3,14,166.1175
3,15,170.37513333333334
3,16,174.5313125
3,17,177.98876470588235
3,18,180.97672222222224
3,19,183.9602105263158
3,20,186.56179999999998
3,21,188.802
3,22,190.88118181818183
3,23,192.82439130434784
3,24,194.6452083333333
3,25,196.24747999999997
3,26,191.99965384615385
3,27,199.09011111111113
3,28,200.44639285714285
3,29,201.72841379310344
3,30,202.8005
3,31,203.7648064516129
3,32,204.850375
3,33,205.8060909090909
3,34,206.46832352941178
3,35,204.67031428571428
4,1,165.135
4,2,165.6795
4,3,164.93633333333335
4,4,157.98975
4,5,158.1886
4,6,164.01116666666667
4,7,164.5482857142857
4,8,165.886
4,9,174.26655555555556
4,10,186.2226
4,11,190.78163636363635
4,12,194.6629166666667
4,13,197.72323076923078
4,14,200.4282142857143
4,15,202.7738
4,16,204.9825625
4,17,206.5091176470588
4,18,208.34133333333332
4,19,209.52031578947367
4,20,210.84314999999998
4,21,211.84014285714284
4,22,212.8908181818182
4,23,214.02826086956523
4,24,214.753375
4,25,215.41244
4,26,216.14626923076924
4,27,216.80744444444443
4,28,217.6055357142857
4,29,218.28189655172412
4,30,218.90966666666665
4,31,219.46429032258064
4,32,219.74859375
4,33,220.28566666666666
4,34,220.5770588235294
4,35,221.00379999999998
5,1,165.328
5,2,165.92
5,3,165.784
5,4,182.38675
5,5,192.6558
5,6,199.59816666666666
5,7,204.80771428571427
5,8,209.068375
5,9,211.81622222222225
5,10,214.0205
5,11,216.2171818181818
5,12,217.22858333333332
5,13,218.32038461538463
5,14,219.6407142857143
5,15,221.00173333333333
5,16,221.98
5,17,222.57211764705883
5,18,223.0601111111111
5,19,223.67684210526318
5,20,224.20905
5,21,224.5677619047619
5,22,225.11781818181817
5,23,225.59091304347828
5,24,226.041125
5,25,226.29256
5,26,226.57103846153845
5,27,227.0064814814815
5,28,227.2703214285714
5,29,227.58689655172412
5,30,227.8476333333333
5,31,227.95887096774194
5,32,228.32228125
5,33,228.5518787878788
5,34,228.83385294117645
5,35,228.86682857142858
6,1,165.54
6,2,199.2165
6,3,210.514
6,4,216.85
6,5,220.3578
6,6,217.9765
6,7,211.838
6,8,211.298625
6,9,214.36755555555555
6,10,226.90890000000002
6,11,227.76209090909092
6,12,228.385
6,13,228.83338461538463
6,14,229.45264285714285
6,15,229.80559999999997
6,16,230.15825
6,17,230.36464705882355
6,18,230.49511111111113
6,19,230.61942105263157
6,20,230.94979999999998
6,21,231.17228571428572
6,22,224.76295454545453
6,23,229.07860869565215
6,24,231.68175
6,25,231.67947999999998
6,26,231.91373076923077
6,27,232.00925925925924
6,28,232.30439285714283
6,29,232.3360344827586
6,30,232.44096666666667
6,31,232.4444516129032
6,32,232.61296875
6,33,232.68300000000002
6,34,232.7481176470588
6,35,232.72719999999998
7,1,231.507
7,2,232.5095
7,3,232.565
7,4,232.62975
7,5,232.882
7,6,233.24216666666666
7,7,233.72857142857143
7,8,233.8825
7,9,234.08544444444445
7,10,233.6706
7,11,233.51936363636364
7,12,233.70325
7,13,234.05107692307695
7,14,234.46342857142855
7,15,234.37546666666668
7,16,234.606625
7,17,234.3744117647059
7,18,234.72011111111112
7,19,234.7378947368421
7,20,234.90120000000002
7,21,232.94714285714286
7,22,225.86072727272727
7,23,234.97734782608694
7,24,234.83266666666665
7,25,235.04592000000002
7,26,235.20938461538464
7,27,235.19248148148145
7,28,234.97253571428573
7,29,235.18472413793106
7,30,235.21776666666668
7,31,235.1725806451613
7,32,235.279
7,33,235.2239090909091
7,34,235.18761764705883
7,35,235.02317142857143
8,1,231.192
8,2,232.536
8,3,231.28766666666667
8,4,233.60125
8,5,233.53759999999997
8,6,233.35933333333332
8,7,233.6177142857143
8,8,233.751
8,9,234.244
8,10,234.3725
8,11,234.60827272727275
8,12,234.4704166666667
8,13,234.8986923076923
8,14,234.75028571428572
8,15,235.03386666666668
8,16,235.2721875
8,17,235.05682352941176
8,18,234.69994444444444
8,19,235.12257894736842
8,20,234.99564999999998
8,21,235.13666666666666
8,22,233.53381818181816
8,23,231.84508695652173
8,24,234.86729166666666
8,25,235.14752000000001
8,26,235.15657692307693
8,27,232.11681481481483
8,28,235.03089285714285
8,29,235.2298620689655
8,30,235.075
8,31,235.07129032258064
8,32,234.99203125
8,33,235.06015151515155
8,34,235.0979117647059
8,35,234.93971428571427
9,1,231.022
9,2,221.782
9,3,218.04966666666667
9,4,232.90925
9,5,233.735
9,6,233.90333333333334
9,7,234.75428571428571
9,8,234.90925
9,9,234.61544444444445
9,10,234.2393
9,11,234.27154545454547
9,12,234.57933333333335
9,13,234.63023076923076
9,14,234.85914285714287
9,15,234.7984
9,16,227.4796875
9,17,233.6306470588235
9,18,234.38944444444445
9,19,234.69836842105263
9,20,234.70784999999998
9,21,234.73738095238096
9,22,234.5662272727273
9,23,234.60882608695655
9,24,234.38995833333334
9,25,234.82348000000002
9,26,234.56353846153843
9,27,234.7514074074074
9,28,234.76660714285717
9,29,234.863
9,30,234.9422
9,31,235.021
9,32,234.87628125
9,33,234.7539696969697
9,34,235.11629411764704
9,35,234.95717142857143
    };
\end{axis}


==> figures/iotlb_sets_ways/a10l_step1_directmapping_vshapeaccessshape.tex <==
\begin{axis}[%
        name=dirv,
        at={($(dirrand.south) + (0cm,-1.75cm)$)},
        anchor=north,
        width=.35\linewidth,
        height=.2625\linewidth,
        scale only axis,
        point meta min=150,
        point meta max=300,
        % xmin=-1,
        % xmax=10,
        xtick={0.5,1.5,...,9.5},
        xticklabels={1,2,4,8,16,32,64,128,256},
        xticklabel style={rotate=90},
        xlabel={Sets},
        xlabel shift=-5pt,
        % ymin=0,
        % ymax=36,
        % ytick={\empty},
        ylabel={Ways},
        axis background/.style={fill=white},
        title style={font=\bfseries,align=center,text width=.3\linewidth,yshift=-5pt},
        title={Direct Mapping V-shape Access},
    ]

    \addplot[%
        surf,
        shader=flat,
        colormap/hot2,
        mesh/rows=10,
    ] table[
        col sep=comma,
        point meta=\thisrow{d}
    ] {
x,y,d
0,1,159.601
0,2,160.2875
0,3,159.937
0,4,160.42425
0,5,160.34759999999997
0,6,160.21766666666662
0,7,160.32485714285716
0,8,160.310875
0,9,160.40733333333333
0,10,161.4783
0,11,160.18481818181817
0,12,160.29533333333333
0,13,160.41884615384615
0,14,161.7295
0,15,161.1379333333333
0,16,160.5313125
0,17,160.7064705882353
0,18,160.42633333333333
0,19,160.62163157894736
0,20,162.01285
0,21,161.5836666666667
0,22,160.32063636363634
0,23,160.28291304347826
0,24,160.2235
0,25,160.22024
0,26,160.38034615384618
0,27,160.35729629629628
0,28,160.29675
0,29,160.2513448275862
0,30,160.28629999999998
0,31,160.339
0,32,160.1785
0,33,160.24418181818183
0,34,160.2480294117647
0,35,160.23742857142858
1,1,160.818
1,2,160.4325
1,3,160.5593333333333
1,4,160.11575
1,5,160.32
1,6,160.08316666666667
1,7,160.30642857142857
1,8,160.2515
1,9,160.16566666666668
1,10,160.2214
1,11,160.11245454545454
1,12,160.22483333333332
1,13,160.17115384615386
1,14,160.21971428571425
1,15,160.18553333333332
1,16,160.16825
1,17,160.22464705882356
1,18,160.14411111111113
1,19,160.14305263157897
1,20,160.19670000000002
1,21,160.0599047619048
1,22,160.19240909090908
1,23,160.17065217391303
1,24,160.24241666666666
1,25,160.2802
1,26,160.13196153846155
1,27,160.27607407407407
1,28,160.87485714285714
1,29,160.23906896551725
1,30,160.25213333333332
1,31,160.29425806451613
1,32,160.0989375
1,33,160.95245454545454
1,34,160.23588235294122
1,35,160.2666857142857
2,1,160.064
2,2,159.9025
2,3,160.039
2,4,159.95825
2,5,160.11520000000002
2,6,159.99316666666667
2,7,160.22242857142857
2,8,159.95375
2,9,159.90644444444445
2,10,159.909
2,11,160.04145454545457
2,12,160.0030833333333
2,13,160.11638461538462
2,14,160.1145
2,15,160.06493333333336
2,16,159.96275
2,17,160.22664705882352
2,18,160.18655555555557
2,19,160.10642105263156
2,20,160.14229999999998
2,21,160.14971428571425
2,22,160.21009090909092
2,23,160.23073913043478
2,24,161.9307916666667
2,25,166.18092
2,26,166.04107692307693
2,27,166.0822962962963
2,28,166.07282142857142
2,29,166.0663448275862
2,30,168.23906666666664
2,31,170.38638709677417
2,32,172.48246875
2,33,174.31715151515152
2,34,175.9830294117647
2,35,177.46305714285714
3,1,165.725
3,2,165.948
3,3,166.21
3,4,165.89775
3,5,165.759
3,6,166.02533333333332
3,7,165.88785714285717
3,8,166.205125
3,9,166.003
3,10,166.00589999999997
3,11,166.0390909090909
3,12,166.124
3,13,166.1003076923077
3,14,165.95114285714283
3,15,170.396
3,16,174.551125
3,17,177.9175882352941
3,18,180.86788888888887
3,19,183.85794736842107
3,20,184.96460000000005
3,21,188.6714761904762
3,22,190.89813636363638
3,23,192.7713043478261
3,24,194.54758333333334
3,25,196.14588
3,26,197.72673076923076
3,27,195.8576666666667
3,28,194.2570357142857
3,29,201.4818620689655
3,30,202.86886666666666
3,31,203.90854838709677
3,32,204.74746875
3,33,205.66309090909093
3,34,206.45244117647061
3,35,207.33057142857143
4,1,166.248
4,2,165.7855
4,3,165.96166666666664
4,4,166.12425
4,5,165.789
4,6,166.01983333333334
4,7,166.044
4,8,174.387875
4,9,175.78988888888887
4,10,176.3615
4,11,188.19336363636364
4,12,194.3683333333333
4,13,197.66830769230768
4,14,200.50485714285716
4,15,202.6392
4,16,204.873875
4,17,206.37876470588236
4,18,208.10416666666666
4,19,209.80210526315793
4,20,210.98844999999997
4,21,211.99671428571426
4,22,212.93063636363635
4,23,213.89539130434784
4,24,214.76579166666667
4,25,215.70904
4,26,216.30265384615385
4,27,216.98025925925927
4,28,217.5914285714286
4,29,218.19989655172415
4,30,218.73043333333334
4,31,219.53493548387098
4,32,220.0525
4,33,220.32233333333335
4,34,220.63976470588236
4,35,221.12345714285715
5,1,166.134
5,2,166.1375
5,3,165.949
5,4,179.694
5,5,188.50179999999997
5,6,199.53033333333335
5,7,204.59085714285715
5,8,208.59775
5,9,211.0771111111111
5,10,213.8692
5,11,215.67863636363634
5,12,217.098
5,13,218.373
5,14,219.6349285714286
5,15,207.75246666666666
5,16,216.771625
5,17,222.4673529411765
5,18,223.25888888888886
5,19,224.0842105263158
5,20,224.5199
5,21,224.97561904761903
5,22,225.4558181818182
5,23,222.24191304347826
5,24,220.86541666666665
5,25,221.442
5,26,226.89503846153843
5,27,227.2457777777778
5,28,227.47514285714286
5,29,227.70693103448275
5,30,227.9651
5,31,228.25309677419358
5,32,228.674
5,33,228.65321212121214
5,34,229.03082352941175
5,35,229.22377142857144
6,1,166.28
6,2,199.687
6,3,209.94966666666667
6,4,205.6715
6,5,220.2104
6,6,222.17766666666668
6,7,223.48042857142858
6,8,225.52025
6,9,226.28922222222218
6,10,227.3212
6,11,227.79854545454546
6,12,228.16158333333334
6,13,228.746
6,14,229.24214285714288
6,15,221.7468
6,16,230.131
6,17,230.28088235294118
6,18,230.42405555555555
6,19,230.7057894736842
6,20,231.001
6,21,230.8674761904762
6,22,231.17872727272726
6,23,231.33517391304346
6,24,219.226875
6,25,229.99852
6,26,232.04103846153845
6,27,232.08014814814814
6,28,232.46103571428574
6,29,232.4289310344828
6,30,232.5044
6,31,232.46635483870966
6,32,232.75528125
6,33,232.67539393939396
6,34,232.7743823529412
6,35,232.84297142857145
7,1,232.303
7,2,225.016
7,3,218.17666666666665
7,4,217.56375
7,5,217.6742
7,6,217.74716666666666
7,7,227.613
7,8,233.912625
7,9,233.59788888888892
7,10,233.43429999999998
7,11,233.56536363636363
7,12,233.7146666666667
7,13,233.83507692307694
7,14,234.1492857142857
7,15,234.3481333333333
7,16,234.165625
7,17,232.12541176470592
7,18,231.75555555555556
7,19,234.53342105263158
7,20,234.67995000000002
7,21,234.83233333333334
7,22,234.75872727272727
7,23,234.65978260869565
7,24,234.77479166666666
7,25,234.81072
7,26,234.8846153846154
7,27,234.90133333333335
7,28,234.79046428571428
7,29,234.9188275862069
7,30,228.13263333333336
7,31,235.1069032258065
7,32,235.01115625
7,33,234.86975757575757
7,34,234.83835294117645
7,35,234.6166
8,1,232.97
8,2,232.4305
8,3,233.09133333333335
8,4,233.6475
8,5,233.4002
8,6,232.5863333333333
8,7,233.51557142857143
8,8,233.953875
8,9,233.78677777777781
8,10,234.0194
8,11,222.54509090909087
8,12,234.76175
8,13,234.7746923076923
8,14,234.5935714285714
8,15,235.09286666666668
8,16,235.0710625
8,17,234.6415882352941
8,18,234.71272222222223
8,19,234.70731578947368
8,20,234.66389999999998
8,21,234.8157619047619
8,22,234.95131818181818
8,23,234.98113043478259
8,24,234.94945833333335
8,25,235.14376000000001
8,26,235.06546153846156
8,27,235.08066666666667
8,28,235.1169642857143
8,29,235.07724137931035
8,30,234.89056666666664
8,31,234.76370967741934
8,32,234.87225
8,33,234.96442424242426
8,34,234.6985294117647
8,35,234.9005142857143
9,1,232.61
9,2,233.056
9,3,232.615
9,4,221.44175
9,5,218.3594
9,6,218.64
9,7,222.2272857142857
9,8,234.748
9,9,234.453
9,10,233.86109999999996
9,11,233.94818181818184
9,12,234.3911666666667
9,13,234.44623076923074
9,14,234.588
9,15,234.35466666666667
9,16,234.348125
9,17,234.4054117647059
9,18,234.3685
9,19,234.45805263157894
9,20,234.4518
9,21,235.06685714285715
9,22,234.3397272727273
9,23,234.4985652173913
9,24,234.52758333333335
9,25,234.51008000000002
9,26,234.53788461538463
9,27,234.4596296296296
9,28,234.59914285714288
9,29,234.70227586206897
9,30,234.7754
9,31,234.92090322580646
9,32,234.66953125
9,33,234.71290909090908
9,34,234.9305
9,35,234.71985714285714
    };
\end{axis}


==> figures/iotlb_sets_ways/a10l_step1_xormapping_directaccessshape.tex <==
\begin{axis}[%
        name=xordir,
        at={($(dirdir.east) + (1.25cm,0cm)$)},
        anchor=west,
        width=.35\linewidth,
        height=.2625\linewidth,
        scale only axis,
        point meta min=150,
        point meta max=300,
        % xmin=-1,
        % xmax=10,
        xtick={0.5,1.5,...,9.5},
        xticklabels={1,2,4,8,16,32,64,128,256},
        xticklabel style={rotate=90},
        % xlabel={Sets},
        % xlabel shift=-5pt,
        % ymin=0,
        % ymax=36,
        % ytick={\empty},
        % ylabel={Ways},
        axis background/.style={fill=white},
        title style={font=\bfseries,align=center,text width=.3\linewidth,yshift=-5pt},
        title={Xor Mapping Direct Access},
    ]

    \addplot[%
        surf,
        shader=flat,
        colormap/hot2,
        mesh/rows=10,
    ] table[
        col sep=comma,
        point meta=\thisrow{d}
    ] {
x,y,d
0,1,161.845
0,2,158.576
0,3,158.45666666666668
0,4,158.3205
0,5,162.87959999999998
0,6,166.2353333333333
0,7,166.31114285714287
0,8,166.317625
0,9,166.38577777777775
0,10,166.5315
0,11,166.34890909090907
0,12,166.23833333333334
0,13,158.27769230769232
0,14,160.31264285714283
0,15,166.2023333333333
0,16,166.2396875
0,17,166.3210588235294
0,18,166.19811111111113
0,19,166.18131578947367
0,20,166.15475
0,21,166.17628571428574
0,22,166.31381818181816
0,23,166.29134782608693
0,24,166.2195
0,25,166.16464000000002
0,26,166.27411538461538
0,27,166.26011111111112
0,28,166.21092857142858
0,29,166.19410344827585
0,30,166.19440000000003
0,31,166.14658064516127
0,32,166.2956875
0,33,166.1238484848485
0,34,166.1870294117647
0,35,166.23991428571426
1,1,165.529
1,2,166.2475
1,3,165.78133333333332
1,4,166.01175
1,5,166.1078
1,6,166.10933333333332
1,7,165.9547142857143
1,8,165.951875
1,9,165.95633333333333
1,10,166.04489999999998
1,11,166.22109090909095
1,12,166.0389166666667
1,13,165.95707692307693
1,14,166.00385714285716
1,15,166.05893333333336
1,16,165.97175
1,17,164.56829411764704
1,18,158.95894444444443
1,19,166.04452631578945
1,20,165.98815
1,21,166.0614285714286
1,22,165.96504545454547
1,23,166.00504347826086
1,24,166.0571666666667
1,25,166.07675999999998
1,26,166.04896153846153
1,27,166.06544444444444
1,28,166.0807857142857
1,29,166.0459655172414
1,30,166.09533333333331
1,31,166.02425806451612
1,32,166.1151875
1,33,166.0199090909091
1,34,166.11644117647057
1,35,166.1424
2,1,165.709
2,2,165.935
2,3,166.02
2,4,166.21875
2,5,165.938
2,6,165.97
2,7,166.25357142857143
2,8,166.11325
2,9,166.02422222222225
2,10,166.01520000000002
2,11,166.00045454545452
2,12,166.11025
2,13,166.03646153846157
2,14,165.82864285714285
2,15,165.86659999999998
2,16,165.9269375
2,17,165.94305882352938
2,18,164.55744444444443
2,19,160.85047368421053
2,20,166.17479999999998
2,21,165.9750952380952
2,22,166.01704545454547
2,23,166.2684347826087
2,24,166.115875
2,25,166.10784
2,26,166.1661923076923
2,27,166.09833333333333
2,28,166.12067857142858
2,29,166.11027586206896
2,30,168.30986666666664
2,31,170.5265483870968
2,32,172.56084375
2,33,174.48166666666665
2,34,176.3379117647059
2,35,177.76905714285718
3,1,166.066
3,2,166.2365
3,3,166.26066666666668
3,4,166.24275
3,5,166.439
3,6,165.93166666666664
3,7,166.2895714285714
3,8,160.182875
3,9,163.66466666666668
3,10,166.11610000000002
3,11,166.1900909090909
3,12,160.98116666666667
3,13,158.17853846153844
3,14,163.61964285714285
3,15,166.99473333333333
3,16,179.0561875
3,17,181.5404117647059
3,18,174.80077777777777
3,19,186.9061052631579
3,20,190.02329999999998
3,21,192.22604761904762
3,22,194.15100000000004
3,23,195.94608695652175
3,24,197.450375
3,25,199.12364000000002
3,26,200.41973076923074
3,27,201.90855555555555
3,28,202.9927142857143
3,29,203.90820689655172
3,30,205.0618333333333
3,31,205.8551612903226
3,32,206.9849375
3,33,207.66972727272727
3,34,208.471
3,35,209.1176
4,1,165.804
4,2,165.795
4,3,166.22566666666668
4,4,166.2145
4,5,166.45219999999998
4,6,166.57183333333333
4,7,175.59071428571428
4,8,183.08275
4,9,188.51211111111112
4,10,193.3998
4,11,186.62481818181817
4,12,188.29341666666664
4,13,200.60446153846152
4,14,205.081
4,15,207.16733333333332
4,16,209.1029375
4,17,210.42729411764705
4,18,211.81388888888887
4,19,212.97305263157892
4,20,214.0875
4,21,215.26604761904764
4,22,215.97168181818182
4,23,216.63165217391307
4,24,217.40354166666668
4,25,218.307
4,26,218.9555
4,27,219.75114814814813
4,28,220.15057142857142
4,29,220.8263793103448
4,30,221.52183333333335
4,31,221.89016129032257
4,32,222.25684375
4,33,222.73618181818182
4,34,222.88088235294117
4,35,223.41157142857142
5,1,165.957
5,2,165.896
5,3,165.51066666666668
5,4,172.95475
5,5,188.8872
5,6,199.60216666666668
5,7,204.97642857142858
5,8,209.245875
5,9,211.59333333333333
5,10,213.9588
5,11,216.1213636363636
5,12,217.69916666666666
5,13,218.90646153846154
5,14,220.0302142857143
5,15,221.11793333333335
5,16,222.09825
5,17,222.77135294117645
5,18,223.43466666666666
5,19,224.25257894736842
5,20,224.77564999999998
5,21,225.15223809523812
5,22,225.3685909090909
5,23,225.83869565217393
5,24,226.216
5,25,226.75815999999998
5,26,226.95526923076926
5,27,227.24807407407405
5,28,227.35310714285717
5,29,227.76327586206898
5,30,227.96390000000002
5,31,228.21032258064514
5,32,228.4544375
5,33,228.58045454545453
5,34,228.64370588235295
5,35,228.86108571428574
6,1,165.311
6,2,199.034
6,3,210.29466666666664
6,4,216.1545
6,5,219.67520000000002
6,6,221.9405
6,7,223.80642857142857
6,8,225.589625
6,9,226.72688888888888
6,10,227.7535
6,11,228.26390909090912
6,12,228.914
6,13,229.42115384615389
6,14,216.96878571428573
6,15,225.7398
6,16,230.404875
6,17,230.42623529411765
6,18,227.6868888888889
6,19,230.92705263157893
6,20,231.0601
6,21,231.46361904761906
6,22,228.03154545454547
6,23,231.77626086956522
6,24,231.8564166666667
6,25,232.02535999999998
6,26,231.91846153846157
6,27,232.06096296296298
6,28,232.00792857142855
6,29,232.28389655172413
6,30,232.3456333333333
6,31,232.32816129032258
6,32,232.648875
6,33,232.5737878787879
6,34,232.6931764705882
6,35,229.07331428571428
7,1,232.199
7,2,233.058
7,3,232.32233333333332
7,4,232.9655
7,5,221.041
7,6,223.99783333333332
7,7,233.50214285714284
7,8,234.035875
7,9,233.7986666666667
7,10,233.71309999999997
7,11,233.49981818181817
7,12,233.4835
7,13,233.45476923076924
7,14,233.72842857142857
7,15,234.1436666666667
7,16,234.1108125
7,17,234.0484117647059
7,18,234.11922222222222
7,19,233.8506842105263
7,20,234.08490000000003
7,21,234.15019047619046
7,22,234.25286363636366
7,23,234.23247826086956
7,24,234.319375
7,25,234.50019999999998
7,26,234.36792307692306
7,27,234.49311111111112
7,28,234.5127857142857
7,29,234.4641724137931
7,30,234.56536666666665
7,31,234.585
7,32,234.4809375
7,33,234.5081212121212
7,34,234.40361764705887
7,35,234.39082857142859
8,1,231.252
8,2,232.399
8,3,232.461
8,4,233.11375
8,5,233.6224
8,6,233.01466666666667
8,7,233.4385714285714
8,8,233.92525
8,9,219.85055555555556
8,10,218.4826
8,11,229.2579090909091
8,12,234.77533333333335
8,13,234.61184615384616
8,14,222.72942857142857
8,15,227.3984
8,16,234.957375
8,17,234.89758823529414
8,18,234.8961111111111
8,19,229.41052631578944
8,20,229.05079999999998
8,21,227.87990476190475
8,22,235.17554545454547
8,23,235.12939130434785
8,24,235.0390833333333
8,25,235.10684
8,26,235.19384615384615
8,27,235.25125925925926
8,28,235.41403571428572
8,29,235.41613793103448
8,30,235.31153333333333
8,31,235.45322580645163
8,32,235.31053125
8,33,235.3290606060606
8,34,235.27120588235294
8,35,235.36785714285713
9,1,231.866
9,2,233.361
9,3,230.49066666666667
9,4,225.839
9,5,233.85739999999998
9,6,234.25016666666664
9,7,234.68142857142857
9,8,234.83175
9,9,234.6548888888889
9,10,234.5482
9,11,234.47354545454547
9,12,234.474
9,13,234.60323076923078
9,14,234.76214285714286
9,15,234.59846666666664
9,16,234.5061875
9,17,234.29658823529414
9,18,234.53722222222225
9,19,234.64736842105265
9,20,234.50240000000002
9,21,234.538
9,22,234.65390909090908
9,23,234.3883913043478
9,24,234.3658333333333
9,25,234.60403999999997
9,26,234.58846153846156
9,27,234.80911111111112
9,28,234.58557142857143
9,29,234.66779310344825
9,30,231.1001
9,31,227.80587096774195
9,32,234.9364375
9,33,234.85963636363635
9,34,234.9331176470588
9,35,234.95877142857142
    };
\end{axis}


==> figures/iotlb_sets_ways/a10l_step1_xormapping_randomaccessshape.tex <==
\begin{axis}[%
        name=xorrand,
        at={($(xordir.south) + (0cm,-1.75cm)$)},
        anchor=north,
        width=.35\linewidth,
        height=.2625\linewidth,
        scale only axis,
        point meta min=150,
        point meta max=300,
        % xmin=-1,
        % xmax=10,
        xtick={0.5,1.5,...,9.5},
        xticklabels={1,2,4,8,16,32,64,128,256},
        xticklabel style={rotate=90},
        % xlabel={Sets},
        % xlabel shift=-5pt,
        % ymin=0,
        % ymax=36,
        % ytick={\empty},
        % ylabel={Ways},
        axis background/.style={fill=white},
        title style={font=\bfseries,align=center,text width=.3\linewidth,yshift=-5pt},
        title={Xor Mapping Random Access},
    ]

    \addplot[%
        surf,
        shader=flat,
        colormap/hot2,
        mesh/rows=10,
    ] table[
        col sep=comma,
        point meta=\thisrow{d}
    ] {
x,y,d
0,1,163.729
0,2,165.3695
0,3,165.70666666666668
0,4,165.652
0,5,166.0518
0,6,165.8501666666667
0,7,165.92857142857142
0,8,165.847125
0,9,165.96044444444445
0,10,166.0205
0,11,166.03427272727274
0,12,165.9764166666667
0,13,166.17492307692305
0,14,166.12657142857142
0,15,166.09946666666667
0,16,165.6431875
0,17,158.06223529411764
0,18,164.63983333333334
0,19,166.05663157894736
0,20,166.13504999999998
0,21,166.03814285714284
0,22,165.98018181818182
0,23,165.9764347826087
0,24,166.09429166666666
0,25,166.05772
0,26,165.96003846153843
0,27,166.043
0,28,166.09910714285715
0,29,166.1038620689655
0,30,166.1211
0,31,166.00829032258068
0,32,166.0515
0,33,166.17439393939395
0,34,166.11785294117647
0,35,166.09882857142858
1,1,165.519
1,2,159.822
1,3,163.54766666666666
1,4,165.69925
1,5,165.61059999999998
1,6,163.76883333333333
1,7,166.14557142857143
1,8,166.02375
1,9,166.02711111111108
1,10,166.0615
1,11,166.0689090909091
1,12,166.10591666666667
1,13,165.85569230769232
1,14,166.0314285714286
1,15,165.94213333333337
1,16,165.992125
1,17,166.07052941176474
1,18,166.06966666666665
1,19,166.1735263157895
1,20,166.19584999999998
1,21,166.11514285714284
1,22,166.20559090909092
1,23,166.13743478260866
1,24,166.16395833333334
1,25,166.13039999999998
1,26,166.12346153846153
1,27,166.19459259259258
1,28,166.1276785714286
1,29,166.12179310344825
1,30,166.0368
1,31,166.10261290322578
1,32,166.10403125
1,33,166.02527272727272
1,34,166.13208823529413
1,35,166.22877142857143
2,1,165.25
2,2,166.096
2,3,166.06466666666668
2,4,166.01975
2,5,162.75459999999998
2,6,158.1885
2,7,158.29271428571425
2,8,165.006
2,9,165.91188888888888
2,10,166.0066
2,11,166.26854545454543
2,12,166.01166666666668
2,13,166.01076923076923
2,14,166.3000714285714
2,15,166.24840000000003
2,16,166.2546875
2,17,166.0176470588235
2,18,166.3082777777778
2,19,166.10905263157895
2,20,166.1371
2,21,166.17819047619048
2,22,166.1217272727273
2,23,166.22113043478262
2,24,165.252125
2,25,166.22372
2,26,166.36946153846156
2,27,166.07729629629628
2,28,166.14771428571427
2,29,166.15648275862068
2,30,168.33896666666666
2,31,170.5308064516129
2,32,172.6318125
2,33,174.47436363636365
2,34,176.26385294117648
2,35,177.80634285714285
3,1,165.66
3,2,165.546
3,3,165.55033333333333
3,4,166.1085
3,5,165.8826
3,6,166.25133333333332
3,7,166.02885714285716
3,8,166.3775
3,9,166.28044444444444
3,10,166.18140000000002
3,11,165.00436363636365
3,12,163.01758333333333
3,13,166.4162307692308
3,14,171.00714285714284
3,15,175.34586666666667
3,16,179.3628125
3,17,182.39323529411766
3,18,185.33544444444445
3,19,187.98568421052636
3,20,190.43025
3,21,192.35690476190476
3,22,194.49563636363635
3,23,195.959652173913
3,24,197.8235
3,25,199.40016
3,26,200.61065384615384
3,27,201.82477777777774
3,28,203.00882142857142
3,29,204.32003448275862
3,30,205.24383333333336
3,31,206.0869677419355
3,32,207.062875
3,33,207.92290909090906
3,34,208.51729411764705
3,35,205.75214285714284
4,1,165.563
4,2,166.5045
4,3,166.043
4,4,166.52875
4,5,166.23579999999998
4,6,166.12283333333332
4,7,175.62971428571427
4,8,183.21975
4,9,188.097
4,10,193.2445
4,11,197.01436363636364
4,12,200.02566666666667
4,13,202.66907692307694
4,14,200.38764285714285
4,15,206.87406666666666
4,16,203.8650625
4,17,208.32929411764704
4,18,211.099
4,19,199.50284210526314
4,20,212.5535
4,21,215.14409523809525
4,22,216.19636363636366
4,23,217.0083043478261
4,24,217.856125
4,25,218.23315999999997
4,26,219.25603846153848
4,27,219.54107407407406
4,28,220.22485714285716
4,29,220.90010344827587
4,30,221.2359
4,31,221.82048387096776
4,32,222.2376875
4,33,222.7911515151515
4,34,223.03035294117646
4,35,223.2823714285714
5,1,165.755
5,2,165.561
5,3,160.692
5,4,172.67025
5,5,183.1488
5,6,188.64533333333333
5,7,204.61871428571428
5,8,208.366375
5,9,211.00388888888887
5,10,213.6825
5,11,215.69945454545453
5,12,217.17775
5,13,218.87476923076923
5,14,219.97607142857143
5,15,220.9171333333333
5,16,221.95225
5,17,222.3824705882353
5,18,223.13305555555556
5,19,223.87952631578946
5,20,224.1832
5,21,224.75061904761904
5,22,225.12386363636364
5,23,225.51778260869565
5,24,225.89341666666667
5,25,226.2876
5,26,226.75526923076922
5,27,226.73755555555556
5,28,227.12960714285717
5,29,227.34079310344825
5,30,227.4839333333333
5,31,227.823
5,32,227.97625
5,33,228.0782121212121
5,34,228.47932352941174
5,35,228.5362285714286
6,1,163.986
6,2,187.6935
6,3,198.09966666666668
6,4,215.98425
6,5,219.9846
6,6,221.97266666666667
6,7,223.727
6,8,225.3575
6,9,212.04933333333332
6,10,212.52809999999997
6,11,219.897
6,12,229.044
6,13,229.34638461538464
6,14,229.9255
6,15,230.10959999999997
6,16,230.303125
6,17,230.69517647058822
6,18,230.79455555555558
6,19,231.0725789473684
6,20,231.1174
6,21,231.31490476190476
6,22,231.81381818181816
6,23,231.78595652173914
6,24,231.88166666666666
6,25,232.01612
6,26,232.07784615384617
6,27,232.1287777777778
6,28,232.20842857142858
6,29,232.471
6,30,232.41039999999998
6,31,232.51990322580644
6,32,231.075375
6,33,232.74403030303034
6,34,232.72914705882351
6,35,232.97702857142855
7,1,231.61
7,2,232.254
7,3,224.63333333333333
7,4,217.7475
7,5,218.0702
7,6,233.04816666666665
7,7,233.43814285714288
7,8,233.790125
7,9,233.70433333333335
7,10,233.5255
7,11,233.39481818181818
7,12,233.74275
7,13,233.37276923076925
7,14,233.77742857142857
7,15,233.81920000000002
7,16,234.0536875
7,17,233.9649411764706
7,18,233.84938888888888
7,19,233.81594736842104
7,20,233.86790000000002
7,21,234.035
7,22,233.97872727272727
7,23,234.1041304347826
7,24,234.4094583333333
7,25,234.30956
7,26,234.31903846153847
7,27,234.2255185185185
7,28,234.495
7,29,234.37651724137933
7,30,234.22896666666668
7,31,234.21622580645163
7,32,234.17115625
7,33,234.0839090909091
7,34,234.2159705882353
7,35,234.3436857142857
8,1,231.531
8,2,232.1725
8,3,233.129
8,4,229.186
8,5,228.4368
8,6,233.00316666666666
8,7,233.65242857142857
8,8,234.22
8,9,234.12833333333333
8,10,234.3666
8,11,234.58654545454544
8,12,234.54675
8,13,234.40323076923076
8,14,234.61864285714285
8,15,234.5728
8,16,234.6975625
8,17,234.80494117647058
8,18,234.81194444444444
8,19,234.9327894736842
8,20,234.90875
8,21,235.01166666666666
8,22,234.8500909090909
8,23,235.0638260869565
8,24,235.042625
8,25,235.18996
8,26,234.86238461538463
8,27,234.90222222222224
8,28,235.07157142857142
8,29,235.0069310344828
8,30,235.14876666666666
8,31,235.2633870967742
8,32,235.10771875
8,33,235.22324242424244
8,34,235.1809705882353
8,35,235.27502857142855
9,1,231.494
9,2,233.1785
9,3,232.37366666666665
9,4,225.59975
9,5,218.3122
9,6,218.70966666666666
9,7,224.26042857142858
9,8,234.907125
9,9,234.67311111111113
9,10,234.42790000000002
9,11,234.42545454545456
9,12,234.85958333333335
9,13,234.40653846153847
9,14,234.13128571428575
9,15,234.20526666666666
9,16,234.4758125
9,17,234.36476470588235
9,18,234.51277777777779
9,19,234.49457894736844
9,20,225.39540000000002
9,21,233.2315238095238
9,22,234.506
9,23,234.45108695652172
9,24,234.6361666666667
9,25,234.54144
9,26,234.59765384615383
9,27,234.596
9,28,234.6744642857143
9,29,234.70886206896552
9,30,234.54196666666667
9,31,234.62119354838708
9,32,234.715
9,33,234.71060606060604
9,34,234.8240294117647
9,35,234.87428571428572
    };
\end{axis}


==> figures/iotlb_sets_ways/a10l_step1_xormapping_vshapeaccessshape.tex <==
\begin{axis}[%
        name=xorv,
        at={($(xorrand.south) + (0cm,-1.75cm)$)},
        anchor=north,
        width=.35\linewidth,
        height=.2625\linewidth,
        scale only axis,
        point meta min=150,
        point meta max=300,
        % xmin=-1,
        % xmax=10,
        xtick={0.5,1.5,...,9.5},
        xticklabels={1,2,4,8,16,32,64,128,256},
        xticklabel style={rotate=90},
        xlabel={Sets},
        xlabel shift=-5pt,
        % ymin=0,
        % ymax=36,
        % ytick={\empty},
        % ylabel={Ways},
        axis background/.style={fill=white},
        title style={font=\bfseries,align=center,text width=.3\linewidth,yshift=-5pt},
        title={Xor Mapping V-shape Access},
    ]

    \addplot[%
        surf,
        shader=flat,
        colormap/hot2,
        mesh/rows=10,
    ] table[
        col sep=comma,
        point meta=\thisrow{d}
    ] {
x,y,d
0,1,166.159
0,2,166.0215
0,3,165.9656666666667
0,4,165.88
0,5,165.964
0,6,165.9768333333333
0,7,166.0815714285714
0,8,166.033625
0,9,165.97488888888887
0,10,166.2359
0,11,165.93236363636365
0,12,164.53758333333334
0,13,158.0653076923077
0,14,164.5035
0,15,166.27559999999997
0,16,166.105875
0,17,166.20964705882355
0,18,166.1183888888889
0,19,166.017
0,20,161.90485
0,21,160.22061904761907
0,22,160.25663636363635
0,23,160.3184347826087
0,24,160.1335
0,25,160.23932000000002
0,26,160.23207692307693
0,27,160.26114814814815
0,28,160.33264285714284
0,29,160.21510344827587
0,30,160.36976666666666
0,31,160.204
0,32,160.2431875
0,33,160.20554545454547
0,34,160.24908823529412
0,35,160.27397142857143
1,1,160.568
1,2,160.1365
1,3,160.38033333333334
1,4,160.47275
1,5,160.1626
1,6,160.22716666666665
1,7,160.36485714285715
1,8,164.348
1,9,166.21044444444445
1,10,166.10770000000002
1,11,166.1922727272727
1,12,164.78691666666666
1,13,166.04146153846156
1,14,165.93592857142858
1,15,166.09706666666668
1,16,166.2139375
1,17,161.7999411764706
1,18,161.52761111111113
1,19,166.13863157894735
1,20,166.24204999999998
1,21,166.26309523809527
1,22,166.13704545454547
1,23,166.0531304347826
1,24,166.126625
1,25,164.03059999999996
1,26,163.4371923076923
1,27,160.4982222222222
1,28,160.2814285714286
1,29,160.2317931034483
1,30,160.2723
1,31,162.0919677419355
1,32,161.003625
1,33,162.18760606060607
1,34,162.8315294117647
1,35,165.3983142857143
2,1,165.152
2,2,166.156
2,3,163.832
2,4,164.6865
2,5,166.5342
2,6,164.70633333333333
2,7,164.96557142857142
2,8,166.5005
2,9,166.27822222222224
2,10,163.7028
2,11,163.29681818181817
2,12,165.55875
2,13,165.05961538461537
2,14,166.34178571428572
2,15,166.38586666666666
2,16,166.253375
2,17,164.1585882352941
2,18,166.35183333333333
2,19,166.16505263157893
2,20,164.957
2,21,166.25571428571428
2,22,166.2001818181818
2,23,164.6977391304348
2,24,160.97845833333335
2,25,160.69012
2,26,165.4026153846154
2,27,166.14711111111112
2,28,166.1020714285714
2,29,166.1565172413793
2,30,168.427
2,31,170.55877419354837
2,32,172.6126875
2,33,174.4767878787879
2,34,176.17064705882356
2,35,177.72202857142855
3,1,166.482
3,2,165.906
3,3,166.027
3,4,166.08875
3,5,166.47320000000002
3,6,166.225
3,7,166.2052857142857
3,8,166.009375
3,9,166.21666666666667
3,10,166.079
3,11,166.19845454545452
3,12,166.2960833333333
3,13,166.13692307692307
3,14,170.88185714285714
3,15,175.24486666666664
3,16,178.793625
3,17,182.09
3,18,184.9761666666667
3,19,187.75257894736842
3,20,190.19754999999998
3,21,192.22380952380954
3,22,194.1182272727273
3,23,196.03530434782607
3,24,197.5415416666667
3,25,199.09807999999998
3,26,200.37715384615385
3,27,201.76062962962965
3,28,202.84985714285716
3,29,203.9606206896552
3,30,204.8568
3,31,206.01590322580645
3,32,206.812875
3,33,207.57154545454546
3,34,208.5009705882353
3,35,206.2947142857143
4,1,166.976
4,2,166.2195
4,3,166.256
4,4,165.95625
4,5,166.1142
4,6,165.99566666666666
4,7,175.56557142857142
4,8,182.788125
4,9,188.33311111111112
4,10,193.1337
4,11,197.11872727272726
4,12,199.92591666666667
4,13,202.45992307692308
4,14,204.89478571428572
4,15,206.95566666666667
4,16,208.6709375
4,17,210.08564705882353
4,18,211.61805555555557
4,19,213.01531578947368
4,20,214.0794
4,21,215.12633333333335
4,22,216.1900909090909
4,23,216.82891304347828
4,24,211.91575
4,25,217.28072
4,26,209.01834615384615
4,27,219.50133333333332
4,28,220.26603571428575
4,29,220.7748275862069
4,30,221.36943333333335
4,31,221.88754838709679
4,32,222.42096875
4,33,222.56139393939392
4,34,222.76173529411764
4,35,218.85240000000002
5,1,166.273
5,2,166.225
5,3,166.0523333333333
5,4,182.476
5,5,192.6104
5,6,199.71
5,7,204.5815714285714
5,8,208.4815
5,9,211.118
5,10,213.5996
5,11,215.54681818181817
5,12,217.1543333333333
5,13,218.67476923076921
5,14,220.04764285714285
5,15,221.01486666666668
5,16,221.8548125
5,17,222.34288235294122
5,18,223.33377777777778
5,19,223.87005263157894
5,20,224.7285
5,21,225.35061904761906
5,22,225.4370909090909
5,23,225.82039130434785
5,24,226.2237916666667
5,25,226.41819999999998
5,26,226.94892307692305
5,27,227.26307407407407
5,28,227.21339285714285
5,29,227.52110344827588
5,30,220.62506666666664
5,31,227.33503225806447
5,32,228.26315625
5,33,228.3341212121212
5,34,228.6198823529412
5,35,228.8594857142857
6,1,166.303
6,2,200.2225
6,3,208.48966666666666
6,4,203.58225
6,5,206.6114
6,6,208.15716666666665
6,7,217.3075714285714
6,8,225.407625
6,9,226.61244444444444
6,10,227.4215
6,11,228.2449090909091
6,12,228.62016666666668
6,13,217.88723076923077
6,14,216.4767857142857
6,15,229.82846666666669
6,16,230.22075
6,17,230.48476470588236
6,18,230.50877777777777
6,19,230.7547894736842
6,20,230.82359999999997
6,21,231.1129523809524
6,22,227.653
6,23,228.29091304347824
6,24,221.74
6,25,231.72072
6,26,231.65046153846154
6,27,232.0664074074074
6,28,231.8642857142857
6,29,232.2276896551724
6,30,232.27246666666667
6,31,232.37051612903224
6,32,232.42671875
6,33,232.6917272727273
6,34,232.58673529411766
6,35,232.81557142857142
7,1,232.295
7,2,232.613
7,3,232.17933333333335
7,4,232.74775
7,5,232.472
7,6,233.3218333333333
7,7,233.8177142857143
7,8,234.09375
7,9,233.8977777777778
7,10,233.74280000000002
7,11,233.66336363636364
7,12,233.9135
7,13,226.68030769230768
7,14,233.958
7,15,234.18813333333335
7,16,234.3325625
7,17,234.31841176470587
7,18,233.91972222222225
7,19,233.81794736842107
7,20,234.07504999999998
7,21,233.5132380952381
7,22,234.09036363636363
7,23,229.10091304347827
7,24,232.3867083333333
7,25,234.42092
7,26,234.3827307692308
7,27,234.4477037037037
7,28,234.46239285714287
7,29,234.415
7,30,234.43640000000002
7,31,234.53506451612904
7,32,234.4128125
7,33,234.5612727272727
7,34,234.3895294117647
7,35,234.48474285714286
8,1,231.824
8,2,232.071
8,3,232.794
8,4,233.55275
8,5,233.4838
8,6,233.0386666666667
8,7,233.97885714285715
8,8,234.2145
8,9,234.485
8,10,234.6558
8,11,234.95818181818183
8,12,234.84216666666666
8,13,234.85307692307694
8,14,234.62114285714287
8,15,234.69553333333332
8,16,234.9716875
8,17,234.9374705882353
8,18,234.977
8,19,235.2216842105263
8,20,235.14525
8,21,234.69980952380953
8,22,235.17172727272725
8,23,234.98
8,24,235.186375
8,25,235.151
8,26,235.04015384615386
8,27,235.22755555555557
8,28,235.03839285714287
8,29,235.21731034482758
8,30,235.18820000000002
8,31,235.2284516129032
8,32,235.37553125
8,33,235.28912121212122
8,34,235.42179411764704
8,35,235.30294285714285
9,1,221.837
9,2,232.6615
9,3,232.94533333333334
9,4,233.92475
9,5,234.37440000000004
9,6,234.616
9,7,234.79414285714284
9,8,234.983
9,9,234.65133333333335
9,10,234.5941
9,11,234.48927272727275
9,12,234.5465
9,13,234.27661538461538
9,14,234.30478571428574
9,15,234.46446666666668
9,16,234.1670625
9,17,234.3149411764706
9,18,224.76327777777777
9,19,232.70784210526315
9,20,234.50189999999998
9,21,234.1587619047619
9,22,234.62568181818182
9,23,234.5501304347826
9,24,234.60166666666666
9,25,233.90628
9,26,231.96761538461539
9,27,232.4265925925926
9,28,232.33389285714287
9,29,232.56951724137932
9,30,232.48153333333332
9,31,232.70490322580645
9,32,232.47275
9,33,232.76145454545454
9,34,232.91208823529414
9,35,233.20528571428574
    };
\end{axis}


==> figures/iotlb_sets_ways/iotlb_sets_ways.tex <==
\begin{tikzpicture}

\input{figures/iotlb_sets_ways/a10l_step1_directmapping_directaccessshape}
\input{figures/iotlb_sets_ways/a10l_step1_directmapping_randomaccessshape}
\input{figures/iotlb_sets_ways/a10l_step1_directmapping_vshapeaccessshape}
\input{figures/iotlb_sets_ways/a10l_step1_xormapping_directaccessshape}
\input{figures/iotlb_sets_ways/a10l_step1_xormapping_randomaccessshape}
\input{figures/iotlb_sets_ways/a10l_step1_xormapping_vshapeaccessshape}

\path (dirv.south) -- node (mapanchor) {} (xorv.south);
\begin{axis}[%
        name=scale,
        at={($(mapanchor.south) + (-.375\linewidth,-1cm)$)},
        anchor=north,
        scale only axis,
        width=0pt,
        height=0pt,
        hide axis,
        point meta min=150,
        point meta max=300,
        colormap/hot2,
        colorbar horizontal,
        colorbar style={xlabel={FPGA Clock Cycles},width=.75\linewidth},
    ]%
    
    \addplot[draw=none] coordinates {(0,0)};
\end{axis}

\end{tikzpicture}

==> figures/its-a10-step1-dir-direct-1-heatmap.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5020.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(660,696){\makebox(0,0)[r]{\strut{}1}}%
      \put(660,984){\makebox(0,0)[r]{\strut{}5}}%
      \put(660,1272){\makebox(0,0)[r]{\strut{}9}}%
      \put(660,1560){\makebox(0,0)[r]{\strut{}13}}%
      \put(660,1848){\makebox(0,0)[r]{\strut{}17}}%
      \put(660,2135){\makebox(0,0)[r]{\strut{}21}}%
      \put(660,2423){\makebox(0,0)[r]{\strut{}25}}%
      \put(660,2711){\makebox(0,0)[r]{\strut{}29}}%
      \put(660,2999){\makebox(0,0)[r]{\strut{}33}}%
      \put(962,440){\makebox(0,0){\strut{}1}}%
      \put(1303,440){\makebox(0,0){\strut{}2}}%
      \put(1644,440){\makebox(0,0){\strut{}4}}%
      \put(1985,440){\makebox(0,0){\strut{}8}}%
      \put(2326,440){\makebox(0,0){\strut{}16}}%
      \put(2666,440){\makebox(0,0){\strut{}32}}%
      \put(3007,440){\makebox(0,0){\strut{}64}}%
      \put(3348,440){\makebox(0,0){\strut{}128}}%
      \put(3689,440){\makebox(0,0){\strut{}256}}%
      \put(4030,440){\makebox(0,0){\strut{}512}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(187,1919){\rotatebox{-270}{\makebox(0,0){\strut{}Ways}}}%
      \put(2496,110){\makebox(0,0){\strut{}Sets}}%
      \csname LTb\endcsname%%
      \put(4587,660){\makebox(0,0)[l]{\strut{}$150$}}%
      \put(4587,939){\makebox(0,0)[l]{\strut{}$160$}}%
      \put(4587,1219){\makebox(0,0)[l]{\strut{}$170$}}%
      \put(4587,1499){\makebox(0,0)[l]{\strut{}$180$}}%
      \put(4587,1779){\makebox(0,0)[l]{\strut{}$190$}}%
      \put(4587,2059){\makebox(0,0)[l]{\strut{}$200$}}%
      \put(4587,2339){\makebox(0,0)[l]{\strut{}$210$}}%
      \put(4587,2619){\makebox(0,0)[l]{\strut{}$220$}}%
      \put(4587,2899){\makebox(0,0)[l]{\strut{}$230$}}%
      \put(4587,3179){\makebox(0,0)[l]{\strut{}$240$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/its-a10-step1-dir-direct-1-heatmap}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pgflibraryshapes.gates.logic.mux.code.tex <==
% Copyright 2008 by Mark Wibrow
% Copyright 2015 by Gabi Sarkis
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgflibrary{shapes.gates.logic}
\usepgflibrary{shapes.gates.logic.IEC}

\pgfkeys{/pgf/.cd,
  mux symbol/.initial=,
}

% Shape mux
%
\pgfdeclareshape{mux}{
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@mux\endcsname{%
    \pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
    %
    \pgfmathloop%
    \ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
    \else%
    \pgfutil@ifundefined{pgf@anchor@mux@input \pgfmathcounter}{%
      \expandafter\xdef\csname pgf@anchor@mux@input \pgfmathcounter\endcsname{%
        \noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
      }%
    }{}%
    \repeatpgfmathloop%
    \ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
    \PackageError{PGF}{A mux must have at least two inputs}{}%
    \fi%
  }%
  \savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
  \saveddimen\invertedradius{%
    \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
  }%
  \saveddimen\outerinvertedradius{%
    \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
    \advance\pgf@x.5\pgflinewidth%
  }
  \savedmacro\dimensions{%
    \pgf@lib@sh@logicgates@dimensions@IEC{mux}%
  }
  \savedanchor\centerpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y-.5\dp\pgfnodeparttextbox%
  }
  \savedanchor\midpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@y{+0.5ex}%
  }
  \savedanchor\basepoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y0pt%
  }
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\midpoint}
  \anchor{mid west}{%
    \dimensions%
    \midpoint%
    \advance\pgf@x-\halfwidth}%
  \anchor{mid east}{%
    \dimensions%
    \midpoint%
    \advance\pgf@x\halfwidth}%
  \anchor{base}{\basepoint}
  \anchor{base west}{%
    \dimensions%
    \basepoint%
    \advance\pgf@x-\halfwidth}%
  \anchor{base east}{%
    \dimensions%
    \basepoint%
    \advance\pgf@x\halfwidth}%
  \anchor{north}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by -\pgfmathresult pt%
  }%
  \anchor{south}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by \pgfmathresult pt%
  }%
  \anchor{east}{\dimensions\centerpoint\advance\pgf@x\halfwidth}%
  \anchor{west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth}%
  \anchor{north east}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{1.155}%
    \advance\pgf@y by -\pgfmathresult pt%
    \advance\pgf@x by \halfwidth%
  }%
  \anchor{north west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth\advance\pgf@y\halfheight}%
  \anchor{south east}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{1.155}%
    \advance\pgf@y by \pgfmathresult pt%
    \advance\pgf@x by \halfwidth%
  }%
  \anchor{south west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth\advance\pgf@y-\halfheight}%
  
  \anchor{select}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by \pgfmathresult pt%
  }%
  
  \anchor{other select}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by -\pgfmathresult pt%
  }%
  
  \anchor{output}{\dimensions\centerpoint\advance\pgf@x\halfwidth} 
  
  \anchor{output}{\dimensions\centerpoint\advance\pgf@x\halfwidth} 
  
  \backgroundpath{%
    \dimensions%
    \pgf@xc\halfwidth%
    \pgf@yc\halfheight%
    \pgfmathaddtolength\pgf@xc{-\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathaddtolength\pgf@yc{-\pgfkeysvalueof{/pgf/outer xsep}}%
    {%
      \pgftransformshift{\centerpoint}%
      
      \pgfmathadd{\pgf@yc}{-1.155\pgf@xc}
      \let\pgf@yd\pgfmathresult
      
      \pgfpathmoveto{\pgfpoint{-\pgf@xc}{-\pgf@yc}}
      \pgfpathlineto{\pgfpoint{-\pgf@xc}{\pgf@yc}}
      \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yd}}
      \pgfpathlineto{\pgfpoint{\pgf@xc}{-\pgf@yd}}
      \pgfpathclose
      
      %
      % Draw inputs.
      %
      \pgf@xc-\halfwidth%
      \advance\pgf@xc-\invertedradius%
      \pgf@yc\halfheight%
      \pgfutil@tempdima2.0\pgf@yc%
      \c@pgf@counta\numinputs%
      \advance\c@pgf@counta1\relax%
      \divide\pgfutil@tempdima\c@pgf@counta%
      \pgfmathloop%
      \ifnum\pgfmathcounter>\numinputs%
      \else%
      \advance\pgf@yc-\pgfutil@tempdima%
      \expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
      {%
        \pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%			
      }%
      \fi%
      \repeatpgfmathloop%
    }%
  }
  
  \foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{mux}}
  
  \anchorborder{%
    \pgfextract@process\externalpoint{}%
    \dimensions%
    \pgfpointadd{\centerpoint}{\pgfpointborderrectangle{\externalpoint}{\pgfqpoint{\halfwidth}{\halfheight}}}%
  }%	
  
}


\endinput


==> tikzlibrarycircuits.logic.mux.code.tex <==
% Copyright 2008 by Till Tantau and Mark Wibrow
% Copyright 2015 by Gabi Sarkis
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{circuits.logic}
\usepgflibrary{shapes.gates.logic.mux}

\tikzset{
  circuit declare symbol = mux,
}

\tikzset{
  set mux graphic={
    circuit symbol open,
    circuit symbol size=width 2.5 height 6,
    shape=mux,
    inner sep=.5ex
  }
}

\endinput

